Smart Meter Privacy with Renewable Energy and an Energy Storage Device

A smart meter (SM) measures a consumer's electricity consumption and reports it automatically to a utility provider (UP) in almost real time. Despite many advantages of SMs, their use also leads to serious concerns about consumer privacy. In this paper, SM privacy is studied by considering the presence of a renewable energy source (RES) and a rechargeable battery (RB), which can be used to partially hide the consumer's energy consumption behavior. Privacy is measured by the information leakage rate, which denotes the average mutual information between the user's real energy consumption and the energy requested from the grid, which the SM reads and reports to the UP. The impact of the knowledge of the amount of energy generated by the RES at the UP is also considered. The minimum information leakage rate is characterized as a computable information theoretic single-letter expression in the two extreme cases, that is, when the battery capacity is infinite or zero. Numerical results are presented for the finite battery capacity case to illustrate the potential privacy gains from the existence of an RB. It is shown that, while the information leakage rate decreases with increasing availability of an RES, larger storage capacity is needed to fully exploit the available energy to improve the privacy.

==> main <==
% Generated by IEEEtran.bst, version: 1.13 (2008/09/30)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{Giaconi:2015}
G.~Giaconi, D.~{G{\"u}nd{\"u}z}, and H.~V. Poor, ``Smart meter privacy with an
  energy harvesting device and instantaneous power constraints,'' in
  \emph{Proc. IEEE Int. Conf. on Commun.}, London, UK, Jun. 2015, pp.
  7216--7221.

\bibitem{Mo:2012}
Y.~Mo, T.-H. Kim, K.~Brancik, D.~Dickinson, H.~Lee, A.~Perrig, and B.~Sinopoli,
  ``Cyber-physical security of a smart grid infrastructure,'' \emph{Proc.
  IEEE}, vol. 100, no.~1, pp. 195--209, Jan. 2012.

\bibitem{smartEnergyGB}
\BIBentryALTinterwordspacing
{Smart Energy GB}. Using a smart meter. [Online]. Available:
  \url{https://www.smartenergygb.org/en/faqs?category=using-a-smart-meter}
\BIBentrySTDinterwordspacing

\bibitem{SMT}
\BIBentryALTinterwordspacing
{Smart Meter Texas}. About us. [Online]. Available:
  \url{https://www.smartmetertexas.com/CAP/public/home/home_about_us.html}
\BIBentrySTDinterwordspacing

\bibitem{Segovia:2011}
\BIBentryALTinterwordspacing
M.~S. R.~Segovia. (2011) Set of common functional requirements of the smart
  meter". [Online]. Available:
  \url{https://ec.europa.eu/energy/sites/ener/files/documents/2011\_10\_smart\_meter\_funtionalities\_report.pdf}
\BIBentrySTDinterwordspacing

\bibitem{EurDir:2009}
{European Union}, ``Directive 2009/72/{EC} of the {European parliament} and of
  the council of 13 {July} 2009 concerning common rules for the internal market
  in electricity and repealing directive 2003/54/{EC},'' \emph{Official J.
  European Union}, vol.~52, no. L211, p. 55–93, Aug. 2009.

\bibitem{Rouf:2012}
I.~Rouf, H.~Mustafa, M.~Xu, W.~Xu, R.~Miller, and M.~Gruteser, ``Neighborhood
  watch: Security and privacy analysis of automatic meter reading systems,'' in
  \emph{Proc. ACM Conf. on Comput. and Commun. Security}, Raleigh, NC, USA,
  Oct. 2012, pp. 462--473.

\bibitem{Hart:1992}
G.~Hart, ``Nonintrusive appliance load monitoring,'' \emph{Proc. IEEE},
  vol.~80, no.~12, pp. 1870--1891, Dec. 1992.

\bibitem{Molina:2010}
A.~Molina-Markham, P.~Shenoy, K.~Fu, E.~Cecchet, and D.~Irwin, ``Private
  memoirs of a smart meter,'' in \emph{Proc. ACM Workshop on Embedded Sensing
  Systems for Energy-Efficiency in Building}, Zurich, Switzerland, Nov. 2010,
  pp. 61--66.

\bibitem{Shaloudegi:2016}
K.~Shaloudegi, A.~Gy{\"{o}}rgy, C.~Szepesv{\'{a}}ri, and W.~Xu, ``{SDP}
  relaxation with randomized rounding for energy disaggregation,''
  \emph{arXiv:1610.09491 [cs.LG]}, Oct. 2016.

\bibitem{Kim:2011}
Y.~Kim, E.~Ngai, and M.~Srivastava, ``Cooperative state estimation for
  preserving privacy of user behaviors in smart grid,'' in \emph{Proc. IEEE
  Int. Conf. on Smart Grid Commun.}, Brussels, Belgium, Oct. 2011, pp.
  178--183.

\bibitem{Bohli:2010}
J.-M. Bohli, C.~Sorge, and O.~Ugus, ``A privacy model for smart metering,'' in
  \emph{Proc. IEEE Int. Conf. on Commun.}, Cape Town, South Africa, May 2010,
  pp. 1--5.

\bibitem{Dwork:2006}
C.~Dwork, ``Differential privacy,'' in \emph{Proc. Int. Colloquium Automata,
  Languages and Programming}, Venice, Italy, Jul. 2006, pp. 1--12.

\bibitem{Backes:2014}
M.~Backes and S.~Meiser, ``Differentially private smart metering with battery
  recharging,'' in \emph{Proc. Int. Workshop Data Privacy Management and
  Autonomous Spontaneous Security}, Egham, UK, Sep. 2014, pp. 194--212.

\bibitem{Sankar:2013}
L.~Sankar, S.~Rajagopalan, S.~Mohajer, and H.~V. Poor, ``Smart meter privacy: A
  theoretical framework,'' \emph{{IEEE} Trans. Inf. Theory}, vol.~4, no.~2, pp.
  837--846, Jun. 2013.

\bibitem{Garcia:2010}
F.~D. Garcia and B.~Jacobs, ``Privacy-friendly energy-metering via homomorphic
  encryption,'' in \emph{Proc. Int. Conf. on Security and Trust Manage.},
  Athens, Greece, Sep. 2010, pp. 226--238.

\bibitem{Li:2011}
F.~Li, B.~Luo, and P.~Liu, ``Secure and privacy-preserving information
  aggregation for smart grids,'' \emph{Int. J. of Security and Networks},
  vol.~6, no.~1, pp. 28--39, Apr. 2011.

\bibitem{Petrlic:2010}
R.~Petrlic, ``A privacy-preserving concept for smart grids,'' in \emph{Proc.
  Sicherheit in vernetzten {Systemen}:18. DFN Workshop}, 2010, p. B1–B14.

\bibitem{Efthymiou:2010}
C.~Efthymiou and G.~Kalogridis, ``Smart grid privacy via anonymization of smart
  metering data,'' in \emph{Proc. IEEE Int. Conf. on Smart Grid Commun.},
  Gaithersburg, MD, USA, Oct. 2010, pp. 238--243.

\bibitem{Kalogridis:2010}
G.~Kalogridis, C.~Efthymiou, S.~Denic, T.~Lewis, and R.~Cepeda, ``Privacy for
  smart meters: Towards undetectable appliance load signatures,'' in
  \emph{Proc. IEEE Int. Conf. on Smart Grid Commun.}, Gaithersburg, MD, USA,
  Oct. 2010, pp. 232--237.

\bibitem{Kalogridis:2011}
G.~Kalogridis, Z.~Fan, and S.~Basutkar, ``Affordable privacy for home smart
  meters,'' in \emph{Proc. IEEE Int. Symposium on Parallel and Distributed
  Process. with Applicat. Workshops}, Busan, Korea, May 2011, pp. 77--84.

\bibitem{Yang:2012}
W.~Yang, N.~Li, Y.~Qi, W.~Qardaji, S.~McLaughlin, and P.~McDaniel, ``Minimizing
  private data disclosures in the smart grid,'' in \emph{Proc. ACM Conf. on
  Comput. and Commun. Security}, Raleigh, NC, USA, 2012, pp. 415--427.

\bibitem{Varodayan:2011}
D.~Varodayan and A.~Khisti, ``Smart meter privacy using a rechargeable battery:
  Minimizing the rate of information leakage,'' in \emph{Proc. IEEE Int. Conf.
  on Acoust., Speech and Signal Process.}, Prague, Czech Republic, May 2011,
  pp. 1932--1935.

\bibitem{Tan:2013JSAC}
O.~Tan, D.~{G{\"u}nd{\"u}z}, and H.~V. Poor, ``Increasing smart meter privacy
  through energy harvesting and storage devices,'' \emph{{IEEE} J. Sel. Areas
  Commun.}, vol.~31, no.~7, pp. 1331--1341, Jul. 2013.

\bibitem{Tan:2017JIFS}
O.~Tan, J.~G\'{o}mez-Vilardeb\'{o}, and D.~G{\"u}nd{\"u}z, ``Privacy-cost
  trade-offs in demand-side management with storage,'' \emph{{IEEE} Trans. Inf.
  Forens. Security}, vol.~12, no.~6, pp. 1458--1469, June 2017.

\bibitem{Li:2016}
S.~Li, A.~Khisti, and A.~Mahajan, ``Privacy-optimal strategies for smart
  metering systems with a rechargeable battery,'' \emph{arXiv:1510.07170v3
  [cs.IT]}, Aug. 2016.

\bibitem{Chin:2016}
J.-X. Chin, T.~T.~D. Rubira, and G.~Hug, ``Privacy-protecting energy management
  unit through model-distribution predictive control,'' \emph{arXiv:1612.05120
  [cs.IT]}, Dec. 2016.

\bibitem{Farokhi:2017}
F.~Farokhi and H.~Sandberg, ``Fisher information as a measure of privacy:
  Preserving privacy of households with smart meters using batteries,''
  \emph{IEEE Trans. on Smart Grid}, Feb. 2017.

\bibitem{Gunduz:2013ICC}
D.~{G{\"u}nd{\"u}z} and J.~G\'{o}mez-Vilardeb\'{o}, ``Smart meter privacy in
  the presence of an alternative energy source,'' in \emph{Proc. IEEE Int.
  Conf. on Commun.}, Budapest, Hungary, Jun. 2013, pp. 2027--2031.

\bibitem{Gomez:2013ISIT}
J.~G\'{o}mez-Vilardeb\'{o} and D.~{G{\"u}nd{\"u}z}, ``Privacy of smart meter
  systems with an alternative energy source,'' in \emph{Proc. IEEE Int. Symp.
  on Inform. Theory}, Istanbul, Turkey, Jul. 2013, pp. 2572--2576.

\bibitem{Gomez:2015TIFS}
J.~{G\'{o}mez-Vilardeb\'{o}} and D.~{G{\"u}nd{\"u}z}, ``Smart meter privacy for
  multiple users in the presence of an alternative energy source,''
  \emph{{IEEE} Trans. Inf. Forens. Security}, vol.~10, no.~1, pp. 132--141,
  Jan. 2015.

\bibitem{tesla}
\BIBentryALTinterwordspacing
{Tesla}. Powerwall 2. [Online]. Available:
  \url{https://www.tesla.com/powerwall}
\BIBentrySTDinterwordspacing

\bibitem{orison}
\BIBentryALTinterwordspacing
Orison. Meet the {Orison} family. [Online]. Available:
  \url{http://orison.energy/}
\BIBentrySTDinterwordspacing

\bibitem{panasonic}
\BIBentryALTinterwordspacing
Panasonic. Residential storage battery system lj-sk84a. [Online]. Available:
  \url{http://www.panasonic.com/au/consumer/energy-solutions/residential-storage-battery-system/lj-sk84a.html}
\BIBentrySTDinterwordspacing

\bibitem{simpliphi}
\BIBentryALTinterwordspacing
{Simpliphi Power}. Phi3.4\textsuperscript{TM} smart-tech battery. [Online].
  Available: \url{http://simpliphipower.com/product/phi3-4-smart-tech-battery/}
\BIBentrySTDinterwordspacing

\bibitem{powervault}
\BIBentryALTinterwordspacing
{Powervault}. Technical specifications. [Online]. Available:
  \url{http://www.powervault.co.uk/technical/technical-specifications/}
\BIBentrySTDinterwordspacing

\bibitem{pecanstreet}
\BIBentryALTinterwordspacing
{Pecan Street}. {Pecan Street Inc. Dataport 2016}. [Online]. Available:
  \url{https://dataport.pecanstreet.org/data/database}
\BIBentrySTDinterwordspacing

\bibitem{intertek}
\BIBentryALTinterwordspacing
{Intertek Testing \& Certification Ltd}. Household electricity survey, a study
  of domestic electrical product usage. [Online]. Available:
  \url{http://randd.defra.gov.uk/Document.aspx?Document=10043_R66141HouseholdElectricitySurveyFinalReportissue4.pdf}
\BIBentrySTDinterwordspacing

\bibitem{dred}
\BIBentryALTinterwordspacing
S.~Akshay. {DRED (Dutch Residential Energy Dataset)}. [Online]. Available:
  \url{http://www.st.ewi.tudelft.nl/\%7Eakshay/dred/}
\BIBentrySTDinterwordspacing

\bibitem{Lichman:2013}
\BIBentryALTinterwordspacing
M.~Lichman, ``{UCI} machine learning repository,'' 2013. [Online]. Available:
  \url{http://archive.ics.uci.edu/ml}
\BIBentrySTDinterwordspacing

\bibitem{microgen}
\BIBentryALTinterwordspacing
{The University of Sheffield - Sheffield Solar}. Microgen database. [Online].
  Available: \url{http://www.microgen-database.org.uk/}
\BIBentrySTDinterwordspacing

\bibitem{Blahut:1972}
R.~Blahut, ``Computation of channel capacity and rate-distortion functions,''
  \emph{{IEEE} Trans. Inf. Theory}, vol.~18, no.~4, pp. 460--473, Jul. 1972.

\bibitem{Arnold:2006}
D.-M. Arnold, H.-A. Loeliger, P.~Vontobel, A.~Kavcic, and W.~Zeng,
  ``Simulation-based computation of information rates for channels with
  memory,'' \emph{{IEEE} Trans. Inf. Theory}, vol.~52, no.~8, pp. 3498--3508,
  Aug 2006.

\bibitem{Deisenroth:2013}
M.~P. Deisenroth, G.~Neumann, and J.~Peters, ``A survey on policy search for
  robotics,'' \emph{Foundations and Trends in Robotics}, vol.~2, pp. 1--142,
  Aug. 2013.

\bibitem{cvx}
\BIBentryALTinterwordspacing
M.~Grant and S.~Boyd, ``{CVX}: Matlab software for disciplined convex
  programming, version 2.1,'' Mar. 2014. [Online]. Available:
  \url{http://cvxr.com/cvx}
\BIBentrySTDinterwordspacing

\bibitem{Cover:1991}
T.~M. Cover and J.~A. Thomas, \emph{Elements of Information Theory}.\hskip 1em
  plus 0.5em minus 0.4em\relax New York, NY, USA: Wiley-Interscience, 1991.

\bibitem{Berger:1971}
T.~Berger, \emph{Rate Distortion Theory: A Mathematical Basis for Data
  Compression}.\hskip 1em plus 0.5em minus 0.4em\relax Englewood Cliffs, NJ:
  Prentice-Hall, 1971.

\bibitem{Gallager:1996}
R.~G. Gallager, \emph{Discrete Stochastic Processes}.\hskip 1em plus 0.5em
  minus 0.4em\relax Springer US, 1996.

\end{thebibliography}

